Differentially Private (Gradient) Expectation Maximization Algorithm with Statistical Guarantees

(Gradient) Expectation Maximization (EM) is a widely used algorithm for estimating the maximum likelihood of mixture models or incomplete data problems. A major challenge facing this popular technique is how to effectively preserve the privacy of sensitive data. Previous research on this problem has already lead to the discovery of some Differentially Private (DP) algorithms for (Gradient) EM. However, unlike in the non-private case, existing techniques are not yet able to provide finite sample statistical guarantees. To address this issue, we propose in this paper the first DP version of (Gradient) EM algorithm with statistical guarantees. Moreover, we apply our general framework to three canonical models: Gaussian Mixture Model (GMM), Mixture of Regressions Model (MRM) and Linear Regression with Missing Covariates (RMC). Specifically, for GMM in the DP model, our estimation error is near optimal in some cases. For the other two models, we provide the first finite sample statistical guarantees. Our theory is supported by thorough numerical experiments.

==> DP_EM.tex <==
\section{Statistical Guarantees of DP Expectation Maximization Algorithm}\label{sec:dpem}
Motivated by idea of the Differentially Private version of Gradient EM algorithm in the previous section, in this section, we will propose a DP variant of EM algorithm. 

Recall that compared with the Gradient EM algorithm, the main difference in EM algorithm is that, in each iteration, we will update the parameter as $\beta^{t+1}=\arg\max_{\beta\in \Omega} Q_n (\beta; \beta^{t})$, where the $Q_n$-function is in (\ref{eq:2}). Thus, to design a DP variant, we need to post-process the parameter $\beta^{t+1}$ via the private 1-dimensional mean estimation of heavy-tailed distribution. Just as the way we post-process the Gradient in Algorithm \ref{alg:2}, we wish to post-process each coordinate of $\beta^{t+1}$ to make it  DP. However, unlike the Gradient EM algorithm where the $\nabla Q_n (\beta; \beta')$ can be written as a sum of $n$ independent components $\frac{1}{n}\sum_{n=1}\nabla q_i (\beta; \beta')$, $\beta^{t+1}$ in  the EM algorithm may not be written as  $n$ independent components (see the Examples below), or even there is no explicit form of $\beta^{t+1}$. Thus, compared with the Assumption \ref{assumption:1}, we need addition assumptions on the form of $\beta^{t+1}=\arg\max_{\beta\in \Omega} Q_n (\beta; \beta^{t})$, which may not hold for some canonical models. 


\begin{assumption}\label{assumption:2}
We assume that for a fixed $\beta'\in \mathcal{B}$, the optimal solution $M_n(\beta')=\arg\max_{\beta\in \Omega} Q_n (\beta; \beta')$ satisfies $M_n(\beta')=\frac{1}{n}\sum_{i=1}^n f_i(\beta')$, where $f_i(\cdot)$ is a function of $y_i$. Moreover, we assume that for each pair $i\neq i'$, $f_i(\beta'), f_{i'}(\beta')$ are independent.  For any fixed $j\in d$, the $j$-th coordinate of $f(\beta)$ \footnote{We denote function $f(\cdot)$ as the function for general $y$. } has bounded second order moment, {\em i.e.,} $\mathbb{E} (f_j(\beta))^2\leq \tau$. We also assume that function $Q(\cdot; \cdot)$ in (\ref{eq:3}) is self-consistent, Lipschitz-Gradient-2($\gamma, \mathcal{B}$), $\upsilon$-strongly concave over some set $\mathcal{B}$. 
\end{assumption}
Note that compared with Assumption \ref{assumption:1}, Assumption \ref{assumption:2} does not need $Q$ to be smooth. However, it needs some unnatural assumptions in the form of $M_n(\beta')$. To show that these assumptions are strong (especially the condition that $f_i, f_{i'}$ are independent for each pair $i\neq i'$), in the following, we will check the three canonical models in the previous section to see whether Assumption \ref{assumption:2} holds. 
\paragraph{Gaussian Mixture Model} For GMM in (\ref{eq:4}), the $Q$ function can be written as 
\begin{equation*}
    Q_n(\beta; \beta')= -\frac{1}{2n}\sum_{i=1}^n \big( w_{\beta'} (y_i) \|y_i-\beta\|_2^2 + [1-  w_{\beta'} (y_i)] \|y_i+\beta\|_2^2 \big). 
\end{equation*}
where $w_\beta(y)=\frac{1}{1+\exp(-\langle \beta, y\rangle/\sigma^2)}$.  Thus, for $ M_n(\beta')=\arg\max_{\beta\in \mathbb{R}^d} Q_n(\beta; \beta')$ we have 
\begin{equation*}
    M_n(\beta')= \frac{2}{n}\sum_{i=1}^n w_{\beta'}(y_i) y_i-\frac{1}{n}\sum_{i=1}^n y_i,
\end{equation*}
Thus $$M_n(\beta')=\frac{1}{n}\sum_{i=1}^n f_i(\beta')$$ for $f_i(\beta')= 2w_{\beta'}(y_i) y_i-y_i $ and for each $i\in [n]$, $f_j$ is independent with others. Later, combing with Lemma \ref{lemma:3} we will show GMM satisfies Assumption \ref{assumption:2}. 

\paragraph{Mixture of Regressions Model}   For MRM in (\ref{eq:5}), the $Q_n$ function can be written as 
\begin{multline*}
    Q_n(\beta;\beta')= \frac{1}{2n} \big(- w_{\beta'}(x_i, y_i)(y-\langle x_i, \beta \rangle)^2\\  + [1-  w_{\beta'} (x_i, y_i)](y+\langle x_i, \beta \rangle)^2 \big),
\end{multline*}
where $w_\beta(x, y)=\frac{1}{1+\exp(-y\langle \beta ,x \rangle/\sigma^2)}$. Thus, for $ M_n(\beta')=\arg\max_{\beta\in \mathbb{R}^d} Q_n(\beta; \beta')$ we have 
\begin{equation*}
     M_n(\beta')= (\frac{1}{n}\sum_{i=1}^n x_i x_i^T )^{-1} \cdot  (\frac{1}{n} \sum_{i=1}^n [2w_{\beta'}(x_i, y_i) -1] y_i x_i). 
\end{equation*}
Thus $M_n(\beta')=\frac{1}{n}\sum_{i=1}^n f_i(\beta')$ for $f_i(\beta')= (\frac{1}{n}\sum_{i=1}^n x_i x_i^T )^{-1} \cdot [2w_{\beta'}(x_i, y_i)-1] y_i x_i$. However, we can see that due to the term of $(\frac{1}{n}\sum_{i=1}^n x_i x_i^T )^{-1}$, for each $i\in [n]$, $f_i$ is dependent with others.  Thus, MRM {\bf does not satisfy} Assumption \ref{assumption:2}. 
\paragraph{Linear Regression with Missing Covariates} For RMC in (\ref{eq:6}),  the $Q_n$ function can be written as  
\begin{equation*}
    Q_n (\beta; \beta')= \frac{1}{n} \sum_{i=1}^n y_i \beta^T m_{\beta'}(x_i^{\text{obs}},y_i)-\frac{1}{2n} \sum_{i=1}^n \beta^T K_{\beta'} (x_i^{\text{obs}},y_i) \beta', 
\end{equation*}
where the functions  $m_{\beta'}(x^{\text{obs}},y), K_{\beta'}  (x^{\text{obs}},y)$ are in (\ref{aeq:4}) and  (\ref{aeq:100}), respectively. Thus, for $ M_n(\beta')=\arg\max_{\beta\in \mathbb{R}^d} Q_n(\beta; \beta')$ we have 
\begin{equation*}
     M_n(\beta')= (\frac{1}{n}\sum_{i=1}^n K_{\beta'} (x_i^{\text{obs}},y_i) )^{-1} \cdot  (\frac{1}{n} \sum_{i=1}^n y_i m_{\beta'}(x_i^{\text{obs}},y_i)). 
\end{equation*}
Thus $M_n(\beta')=\frac{1}{n}\sum_{i=1}^n f_i(\beta')$ for $f_i(\beta')=  (\frac{1}{n}\sum_{i=1}^n K_{\beta'} (x_i^{\text{obs}},y_i) )^{-1}  (y_i m_{\beta'}(x_i^{\text{obs}},y_i))$. However, we can see that due to the term of $(\frac{1}{n}\sum_{i=1}^n K_{\beta'} (x_i^{\text{obs}},y_i) )^{-1} $, for each $i\in [n]$, $f_i$ is dependent with others.  Thus, RMC {\bf does not satisfy} Assumption \ref{assumption:2}. 

From the previous models, we can see that two of them do not satisfy the condition of $f_i$ is independent with others. We note that this assumption is necessary for our analysis of statistical guarantees, since we will use the private 1-dimensional mean estimator, which needs the i.i.d assumption on the samples. Thus, from this point of  view, we can see that our DP  Gradient EM algorithm needs to be presented before the DP EM algorithm. 

\subsection{DP EM Algorithm}
Next we will detail our DP EM algorithm and provide its statistical guarantee under Assumption \ref{assumption:2}, see Algorithm \ref{alg:3} for details. The key idea is that in each iteration, instead of post-processing the $j$-th coordinate of the gradient $\nabla q_i(\beta^{t-1}, \beta^{t-1})$, we will post-process $j$-th coordinate of the term $f_i(\beta^{t-1})$, {\em i.e.,} $f_{i,j}(\beta^{t-1})$ via the previous private 1-dimension mean estimator. 
\begin{algorithm*}[!ht]
	\caption{DP EM Algorithm} \label{alg:3}
	$\mathbf{Input}$: $D=\{y_i\}_{i=1}^n\subset \mathbb{R}^d$, privacy parameters $\epsilon, \delta$, $Q(\cdot; \cdot)$ and its $f_i(\cdot)$ in Assumption \ref{assumption:2},  initial parameter $\beta^0\in \mathcal{B}$, $\tau$ which satisfies Assumption \ref{assumption:2}, the number of iterations $T$ (to be specified later),  and failure probability $\zeta$. 
	\begin{algorithmic}[1]
    \State Let $\tilde{\epsilon}= \sqrt{\log \frac{1}{\delta}+\epsilon}-\sqrt{\log \frac{1}{\delta}}$, $s={\frac{\sqrt{n\tau\tilde{\epsilon}}}{2\log \frac{d}{\zeta}}}$, $\beta=\sqrt{\log \frac{d}{\zeta}}$. 
    \For {$t=1, 2, \cdots, T$}
    \State For each $j\in [d]$, calculate the robust estimator by (\ref{eq:9})-(\ref{eq:13}) and add Gaussian noise, that is 
    \begin{multline}
        g_j^{t-1}(\beta^{t-1})= \frac{1}{n}\sum_{i=1}^n \left( f_{i,j}(\beta^{t-1})\big(1-\frac{f^2_{i,j}(\beta^{t-1})}{2s^2\beta}\big)- \frac{f^3_{i,j}(\beta^{t-1})}{6s^2}\right)+\frac{s}{n}\sum_{i=1}^n\hat{C}\left(\frac{f_{i,j}(\beta^{t-1})}{s}, \frac{|f_{i,j}(\beta^{t-1})|}{s\sqrt{\beta}}\right)+ Z_{j}^{t-1},
    \end{multline}
    where $f_{i,j}(\beta^{t-1})$ is the $j$-th coordinate of $f_{i}(\beta^{t-1})$ and $Z_{j}^{t-1}\sim \mathcal{N}(0, \sigma^2)$ with $\sigma^2= \frac{16s^2 dT}{9 n^2\tilde{\epsilon}^2}=\frac{4dT\tau}{9n\beta^2\tilde{\epsilon}}$.
    \State Let vector $\tilde{f}(\beta^{t-1})\in \mathbb{R}^d$ to denote  $\tilde{f}(\beta^{t-1})=(g_1^{t-1}(\beta^{t-1}), g_2^{t-1}(\beta^{t-1}), \cdots, g_d^{t-1}(\beta^{t-1}))$. 
    \State Update
        $\beta^{t}=\tilde{f}(\beta^{t-1}). $
    \EndFor
	\end{algorithmic}
\end{algorithm*}
 We can easily show Algorithm \ref{alg:3} is $(\epsilon, \delta)$-DP. 
\begin{theorem}[Privacy guarantee]
For any $0< \epsilon, \delta<1 $,  Algorithm \ref{alg:2} is $(\epsilon, \delta)$-DP. 
\end{theorem}
\begin{proof}
The proof is almost the same as  that of Theorem \ref{theorem:2}; we thus omit it here. 
\end{proof}
As in Theorem \ref{theorem:3}, in the following, we will show the statistical guarantee for the models under the Assumption \ref{assumption:2}, if the initial parameter $\beta^0$ is close enough to the underlying parameter $\beta^*$.

\begin{theorem}[Statistical guarantee of Algorithm \ref{alg:3}]\label{theorem:30} Let the parameter set $\mathcal{B}=\{\beta: \|\beta-\beta^*\|_2\leq R \}$ for $R=\kappa \|\beta^*\|_2$ for some constant $\kappa \in (0, 1)$.  Assume that  Assumption \ref{assumption:2} holds for parameters $\gamma, \mathcal{B},  v, \tau $ satisfying the condition of $1-2\frac{v-\gamma}{v+\mu} \in (0, 1)$. Also, assume that $\|\beta^0-\beta^*\|_2\leq \frac{R}{2}$, $n$ is large enough so that 
\begin{equation}
%\vspace{-0.05in}
\tilde{\Omega}( (\frac{v}{v-\gamma})^2 \frac{d^2\tau T \sqrt{\log \frac{1}{\delta}} \log \frac{1}{\zeta} }{\epsilon R^2})\leq n.  
\end{equation}
Then with probability at least $1-\zeta$,  we have for all $t\in [T]$, $\beta^t\in \mathcal{B}$. If it holds and if we take $T=O(\frac{v}{v-\gamma}\log n )$, then we have 
\begin{equation}
%\vspace{-0.05in}
    \|\beta^T-\beta^*\|_2\leq \tilde{O}\big(R\sqrt{\frac{v}{(v-\gamma)^3}} \frac{d \sqrt[4]{\log \frac{1}{\delta}}\log \frac{1}{\zeta}\sqrt{\tau}}{\sqrt{n \epsilon}} \big), 
\end{equation}
where the $\tilde{O}$-term and $\tilde{\Omega}$-term  omit $\log d$, $\log n$ and other factors. 
%(see Appendix for the explicit form of the result). 

\end{theorem}
\begin{proof}[{\bf Proof of Theorem \ref{theorem:30}}]
For each iteration we denote $M(\beta^{t-1})=\arg\max Q(\beta; \beta^{t-1})$, by the strongly concavity of $Q(\beta; \beta^*)$ we have 
\begin{multline*}
    \langle \nabla Q(M(\beta^{t-1}); \beta^*)- \nabla Q(\beta^*; \beta^*), M(\beta^{t-1})-\beta^*\rangle \\ \geq v \|M(\beta^{t-1})-\beta^*\|_2^2. 
\end{multline*}
On the other hand, by the Lipschitz-Gradient condition and the  assumption of $M(\beta^{t-1}), \beta^{t-1}\in \mathcal{B}$, we have 
\begin{multline*}
       \langle \nabla Q(M(\beta^{t-1}); \beta^*)-\nabla Q(M(\beta^{t-1}); \beta^{t-1}), \beta^*- M(\beta^{t-1})\rangle \\ \leq \gamma \|\beta^{t-1}-\beta^*\|_2\| \beta^*- M(\beta^{t-1})\|_2.
\end{multline*}
Also by the optimality of $M(\beta^{t-1})$ we have 
\begin{multline*}
   \langle \nabla Q(M(\beta^{t-1}); \beta^*)- \nabla Q(\beta^*; \beta^*), M(\beta^{t-1})-\beta^*\rangle  \\ \leq     \langle \nabla Q(M(\beta^{t-1}); \beta^*)-\nabla Q(M(\beta^{t-1}); \beta^{t-1}), \beta^*- M(\beta^{t-1})\rangle.
\end{multline*}
Thus, we have 
\begin{equation*}
    v \|M(\beta^{t-1})-\beta^*\|_2^2\leq \gamma \|\beta^{t-1}-\beta^*\|_2\|_2 \beta^*- M(\beta^{t-1})\|_2.
\end{equation*}
That is, $\|M(\beta^{t-1})-\beta^*\|_2\leq \frac{\gamma}{v}\|\beta^{t-1}-\beta^*\|_2$. Next, we will bound the term of $\|\beta^t-M(\beta^{t-1})\|_2$. 

Under the assumption that $f_i$ is independent with others, just as almost the same as in (\ref{aeq:7})-(\ref{aeq:9}) via Lemma \ref{lemma:2}, we have that with probability at least $1-\zeta$,
\begin{equation*}
   \|\beta^t-M(\beta^{t-1})\|_2=  \|\tilde{f}(\beta^{t-1})-M(\beta^{t-1})\|_2\leq O(\frac{ d\sqrt{\tau T\log \frac{d}{\zeta}}}{\sqrt{\beta n\tilde{\epsilon}}}). 
\end{equation*}
Thus, we have with probability at least $1-\zeta$
\begin{equation*}
    \|\beta^t-\beta^*\|_2\leq \frac{\gamma}{v}\|\beta^{t-1}-\beta^*\|_2+ O(\frac{ d\sqrt{\tau T\log \frac{d}{\zeta}}}{\sqrt{\beta n\tilde{\epsilon}}}). 
\end{equation*}
Since we need to make $\beta^t\in \mathcal{B}$, this will be true under the assumption that 
\begin{equation*}
    O(\frac{ d\sqrt{\tau T\log \frac{d}{\zeta}}}{\sqrt{\beta n\tilde{\epsilon}}}) \leq \frac{v-\gamma}{v} R.
\end{equation*}
If this holds, then we have with probability at least $1-T\zeta$
\begin{equation*}
     \|\beta^t-\beta^*\|_2\leq (\frac{\gamma}{v})^T R+ O(\frac{v}{v-\gamma}\frac{ d\sqrt{\tau T\log \frac{d}{\zeta}}}{\sqrt{\beta n\tilde{\epsilon}}}), 
\end{equation*}
Taking $T=O(\frac{v}{v-\gamma}\log n)$ and $\tilde{\epsilon}=O(\frac{\epsilon}{\sqrt{\log \frac{1}{\delta}}})$, we have the result. 
\end{proof}
Comparing with Theorem \ref{theorem:30} and Theorem \ref{theorem:3}, if we omit other factors instead of $n, d, \epsilon, \delta$, we can see that the two error bounds are asymptotically the same. 

In the following we will apply our general framework to the GMM model in (\ref{eq:4}). Just the same as in  Theorem \ref{theorem:4}, we will first show that $f_j(\beta)$ has a  bounded second order moment. 
\begin{lemma}\label{alemma:200}
Consider the function $f(\cdot)$ in GMM. Then, for each $j\in [d]$ we have 
\begin{equation*}
    \mathbb{E} f^2_j(\beta) \leq O(\|\beta^*\|_\infty^2+\sigma^2). 
\end{equation*}
\end{lemma}
\begin{proof}[{\bf Proof of Lemma \ref{alemma:200} }]
To prove Lemma \ref{alemma:200}, we need a stronger lemma. 
\begin{lemma}\label{alemma:90}
The $j$-the coordinate of $f(\beta)$ is $\xi$-sub-exponential with 
%%\vspace{-0.1in}
\begin{equation}
    \xi = C_1\sqrt{\|\beta^*\|_\infty^2+\sigma^2},
\end{equation}
where $C_1$ is some absolute constant. Also, for fixed $j\in [d]$, each $f_{i,j}(\beta)$, where $i\in [n]$, is independent with others.
\end{lemma}
If Lemma \ref{alemma:90} holds, then by Lemma \ref{alemma:2} we can get Lemma \ref{alemma:200}. 
\end{proof}
\begin{proof}[Proof of Lemma \ref{alemma:90}]
The proof is almost the same as that  of Lemma \ref{lemma:4}.


It is oblivious that each $f_{i}(\beta)$, where $i\in [n]$, is independent with others. Next, we prove the property of sub-exponential for each coordinate. 

Note that $$f_{j}(\beta)= [2w_\beta(y)-1]y_{j},$$ and $$\mathbb{E}_{Y}f_{i}(\beta)= \mathbb{E}_{Y}(2w_\beta(Y)Y_j-Y_j).$$ 


By the symmetrization lemma in Lemma \ref{alemma:7}, we have the following for any $t>0$
\begin{equation}
    \mathbb{E}\{\exp(t|[f_{j}(\beta)-\mathbb{E}f_{j}(\beta)]|)\}\leq  \mathbb{E}\{\exp(t|\epsilon [2w_\beta(y)-1]y_{j}|)\},
\end{equation}
where $\epsilon$ is a Rademacher random variable. 

Next, we use Lemma \ref{alemma:8} with $f(y_{j})=y_{j}$, $\mathcal{F}=\{f\}$, $\phi(v)=[2w_\beta(y)-1]v$ and $\phi(v)=\exp(u\cdot v)$. It is easy to see that $\phi$ is 1-Lipschitz. Thus,  by Lemma \ref{alemma:8} we have
\begin{equation}
    \mathbb{E}\{\exp(t|\epsilon [2w_\beta(y)-1]y_{j}|)\}\leq \mathbb{E}\{\exp[2t|\epsilon y_{j}|]\}. 
\end{equation}

By the formulation of the model, we have $y_{ j}=z \beta^*_{j}+v_{j}$, where $z$ is a Rademacher random variable and $v_{j}\sim \mathcal{N}(0, \sigma^2)$. It is easy to see that $y_{j}$ is sub-Gaussian and 
\begin{multline}
        \|y_{j}\|_{\psi_2}=\|z\cdot \beta^*_j+v_{j}\|_{\psi_2} \leq C\cdot \sqrt{\|z\cdot \beta_j\|^2_{\psi_2}+\|v_{j}\|^2_{\psi_2}}\\ \leq C'\sqrt{|\beta_j^*|^2+\sigma^2}
\end{multline}

for some absolute constants $C, C'$, where the last inequality is due to the facts that $\|z_j\beta_j^*\|_{\psi_2}\leq |\beta_j^*|$ and $\|v_{i,j}\|_{\psi_2}\leq C''\sigma^2$ for some $C''>0$. 

Since $|\epsilon y_{j}|=|y_{j}|$, $\|\epsilon y_{j}\|_{\psi_2}=\|y_{j}\|_{\psi_2}$ and $\mathbb{E}(\epsilon y_{j})=0$, by Lemma 5.5 in \citep{vershynin2010introduction} we have that  for any $u'$ there exists a constant $C^{(4)}>0$ such that 
\begin{equation}
    \mathbb{E}\{\exp(u' \cdot \epsilon \cdot y_{j})\}\leq \exp(u'^2\cdot C^{(4)} \cdot (|\beta|_j^2+\sigma^2)). 
\end{equation}
Thus, for any $t>0$ we get
\begin{equation}
      \mathbb{E}\{\exp(2t\cdot |\epsilon \cdot y_{j}|)\}\leq 2\exp(t^2\cdot C^{(5)}\cdot (|\beta|_j^2+\sigma^2))
\end{equation}
for some constant $C^{(5)}$. 
Therefore, in total we have the following  for some constant $C^{(6)}>0$
\begin{multline}
      \mathbb{E}\{\exp(t|[f_{j}(\beta)-\mathbb{E}f_{j}(\beta)]|)\} \leq \exp(t^2\cdot C^{(6)}\cdot (|\beta|_j^2+\sigma^2))\\ \leq \exp(t^2\cdot C^{(6)}\cdot (\|\beta^*\|_\infty^2+\sigma^2)).
\end{multline}
    

Combining this with Lemma \ref{alemma:4} and the definition,  we know that  $f_{j}(\beta)$ is $O(\sqrt{\|\beta^*\|_\infty^2+\sigma^2})$-sub-exponential. 
\end{proof}
Thus, combining with Lemma \ref{lemma:3}, Lemma \ref{alemma:200} and Theorem \ref{theorem:30} we have asymptotically the same result as in Theorem \ref{theorem:4}. We omit the details here. 





\iffalse
\begin{figure*} \centering
 \subfigure[$n=2000,d = 10$\label{Gmm_budget_alg3}]
 {\includegraphics[trim=0.05in 0 0.8in 0.7in,clip,width=2.2in]{GMM_multi_budget_alg3.png}}
\subfigure[$n=2000, \epsilon = 0.5$ \label{Gmm_dim_alg3}]
  {\includegraphics[trim=0.05in 0 0.8in 0.7in,clip,width=2.2in]{GMM_dim_alg3.png}}
     \subfigure[$d=10, \epsilon =0.5$\label{Gmm_samples_alg3}]
  {\includegraphics[trim=0.05in 0 0.8in 0.7in,clip,width=2.2in]{GMM_sample_alg3.png}}
 \caption{ Estimation error of GMM w.r.t privacy budget $\epsilon$, data dimension $d$ and data size $n$ (we set $\beta \coloneqq \beta^T $ with $T = 5$)} \label{fig:comp_gmm_alg3}
\end{figure*}


\begin{figure*} \centering
 \subfigure[$n=2000,d = 10$\label{Gmm_budget_2_alg3}]
 {\includegraphics[trim=0.05in 0 0.8in 0.6in,clip,width=2.2in]{GMM_multi_budget_2_alg3.png}}
\subfigure[$n=2000, \epsilon = 0.5$ \label{Gmm_dim_2_alg3}]
  {\includegraphics[trim=0.05in 0 0.8in 0.7in,clip,width=2.2in]{GMM_dim_2_alg3.png}}
     \subfigure[$d=10, \epsilon =0.5$\label{Gmm_samples_2_alg3}]
  {\includegraphics[trim=0.05in 0 0.8in 0.7in,clip,width=2.2in]{GMM_sample_2_alg3.png}} %\vspace{-0.1in}
 \caption{  Estimation error of GMM w.r.t privacy budget $\epsilon$, data dimension $d$, data size $n$ and iteration $t$} \label{fig:comp_gmm_2_alg3}
\end{figure*}
\fi 






==> chapter_exp.tex <==





